Towards a Formal Framework for Partial Compliance of Business Processes

Binary "YES-NO" notions of process compliance are not very helpful to managers for assessing the operational performance of their company because a large number of cases fall in the grey area of partial compliance. Hence, it is necessary to have ways to quantify partial compliance in terms of metrics and be able to classify actual cases by assigning a numeric value of compliance to them. In this paper, we formulate an evaluation framework to quantify the level of compliance of business processes across different levels of abstraction (such as task,trace and process level) and across multiple dimensions of each task (such as temporal, monetary, role-, data-, and quality-related) to provide managers more useful information about their operations and to help them improve their decision making processes. Our approach can also add social value by making social services provided by local, state and federal governments more flexible and improving the lives of citizens.

==> images/designTime/complaintHandling.tex <==
%!TEX root = ../paper.tex

{
\begin{tikzpicture}[
ProcessNode/.style={processNode,font=\scriptsize,rounded corners=3pt,text width=3em,minimum height=2.8em},
GatewayNode/.style={gatewayNode},
EventNode/.style={eventNode},
placeHolderNode/.style={draw=none,minimum width=#1},
taskId/.style={draw=none,font=\scriptsize,text centered,inner sep=3pt},
lbl/.style={Label,font=\tiny},
conditionLabel/.style={lbl,yshift=-1.9em,text width=30,anchor=north,below},
decisionLabel/.style={lbl,text centered},
l/.style={->,rounded corners=5pt,shorten >=0pt,shorten <=0pt},
]

\matrix (base) [draw=none,
  column sep=7pt,row sep=0pt,
] {
\node (start) [MessageStartEvent,label={[lbl]below:Compliant}] {} ; 
  & \node (g1) [GatewayNode,ExclusiveGateway] {} ;
  & [.7em] \node (oralComplaint) [ProcessNode] {Acknow Oral} ;
  & \node (g2) [GatewayNode,ExclusiveGateway] {} ;
  & \node (resolved) [ProcessNode] {Resolve Complaint} ;
  & \node (g3) [GatewayNode,ExclusiveGateway,label={[lbl]above:Resolve in 7 days}] {} ; \\
&& \node (writtenComplaint) [ProcessNode] {Acknow written within 2 days} ;
  & & & \node (escalateComplaint) [ProcessNode] {Escalate complaint} ;
  & \node (g4) [GatewayNode,ExclusiveGateway,label={[lbl]above:Resolve in 3 days}] {} ;
  & [1cm] \node (g5) [GatewayNode,ExclusiveGateway] {} ;
  & \node (end) [EndEvent] {} ; \\
&&&&& & \node (g6) [GatewayNode,ExclusiveGateway] {} ;
  & [1cm] \node (g7) [GatewayNode,ExclusiveGateway] {} ; \\
};

\node [lbl,anchor=east] at (g6.west) {arbitration require?} ;
\node (arbitration) [ProcessNode,anchor=north,yshift=-.5em] at ($(g6.south)!.5!(g7.south)$) {Seek arbitration} ; 

\foreach \n/\l [remember=\n as \lastn (initially start)] in {g1/} {
  \draw [l,->] (\lastn) -- node [lbl] {\l} (\n) ;
}

\foreach \n/\l [remember=\n as \lastn (initially g2)] in {resolved/,g3/,escalateComplaint/No,g4/,g5/Yes,end/} {
  \draw [l,->] (\lastn) -- node [lbl] {\l} (\n) ;
}


\draw [l,->] (g4) -- node [lbl,swap] {No} (g6) ;
\draw [l,->] (g6) -- node [lbl] {No} (g7) ;
\draw [l,->] (g7) -- (g5) ;


\draw [l,->] (g1) -- node [lbl] {oral} (oralComplaint) ;
\draw [l,->] (oralComplaint) -- (g2);

\draw [l,->] (g1) |- node [lbl,swap] {wirtten} (writtenComplaint) ;
\draw [l,->] (writtenComplaint) -| (g2) ;

\draw [l,->] (g3) -| (g5) ;

\draw [l,->] (g6) |- node [lbl,swap] {Yes} (arbitration) ;
\draw [l,->] (arbitration) -| (g7) ;

\end{tikzpicture}
}

\endinput


==> images/designTime/frag1.tex <==
%!TEX root = ../paper.tex

{
\begin{tikzpicture}[font=\tiny\sffamily,
  node distance=.4 and .9,
  every node/.style={text centered,inner sep=5pt,draw},
  l/.style={->,rounded corners=5pt},
  lbl/.style={auto,draw=none,font=\tiny,text width=25,inner sep=2pt},
  classlbl/.style={anchor=south,rotate=90,draw=none,font=\footnotesize,minimum height=2.2em,minimum width=55,xshift=0pt},
  annotationNode/.style={ellipse,draw,font=\footnotesize\sffamily},
  processEvent/.style={rounded corners=3pt,text width=20,minimum height=2.5em,minimum width=1em,,fill=blue!10},
  wrapper/.style={inner sep=4pt,draw},
  classname/.style={anchor=south,rotate=90,draw=none},
  classwrapper/.style={draw=none,inner sep=8pt,anchor=west},
  processwrapper/.style={inner sep=0pt,draw},
  whitecir/.style={circle,text width=6pt,inner sep=0pt,draw,fill=white,solid},
]
%=====================
% CONTRACTOR SIDE
%=====================
\matrix (base) [draw=none,
  column sep=7pt,row sep=10pt
  % nodes={draw},
  % nodes={text width=40},
] {
  & & & \node (p2c) [processEvent,text width=23] {Draw New Conditions}; 
  & \node (PP4) [processEvent] {Receive\\Approval}; 
  & \node (gate4)[ExclusiveGateway]{}; \\
  & & \node (gateU2) [ExclusiveGateway] {}; 
  & & & \node (gate2)[ExclusiveGateway]{}; \\
  & & \node (gateU1) [ExclusiveGateway] {}; \\
\node (start) [MessageStartEvent] {}; 
  & \node (p1) [processEvent,minimum width=10] {Analyse Request};
  & \node (gate1) [ExclusiveGateway] {};\\ 
  & & &\node (p3) [processEvent,text width=30] {Accept as\\ Amendment};
  & \coordinate (c1);\\ 
};
\node (E1) [TerminateEndEvent,right=of gate2,xshift=-.6cm]{}; 
\node (gate3)[ExclusiveGateway,right=of E1,xshift=-.8cm]{};
\node (p5) [processEvent,right=of gate3,xshift=-.5cm] {Amend\\Contract};
\node (End) [EndEvent,right=of p5,xshift=-.5cm] {};

\node [lbl,anchor=west,align=left] at (gate1.east) {Type};
\node [lbl,anchor=west,text width=40,align=center] at (gateU2.north) {New\\Conditions};
\node [lbl,anchor=west] at (gate4.north) {Approved?};
\node [lbl,anchor=north] at (E1.south) {End};
\node [lbl,anchor=north] at (start.south) {Received Request};
\node [lbl,anchor=north] at (End.south) {End};

\draw [l] (gate1)|- node [lbl,swap]{Minor Request} (p3);
\draw [l] (gate1) -- node [lbl,swap,text width=30] {Major Request} (gateU1);
\draw [l] (gateU1) -- node [lbl] {Accept} (gateU2);
\draw [l] (gateU2) |- node [lbl] {Yes} (p2c);


\foreach \n [remember=\n as \lastn (initially start)] in {p1,gate1} {
  \draw [l] (\lastn) -- (\n);
}

\foreach \n/\l [remember=\n as \lastn (initially gate3)] in {p5,End} {
  \draw [l] (\lastn) -- (\n);
}
\draw [l] (p2c)--(PP4);
\draw [l] (PP4)--(gate4);
\draw [l] (gateU2)-- node [lbl,swap,xshift=1.2cm]{No}(gate2);
\draw [l] (gate4)-- node [lbl,swap,rotate=90,yshift=.2cm,xshift=.5cm]{No}(gate2);
\draw [l] (gate2)--(E1);
\draw [l] (p3)-|(gate3);
\draw [l] (gate4)-|node [lbl,xshift=-.8cm,yshift=-.7cm]{Yes}(gate3);
\draw [l] (gateU1)-|node [lbl,yshift=-.1cm]{Reject}(gate2);

% \node (cw1) [classwrapper,fit=(base)(p2)(p3)(minorrequest)] {};
\node (cw1) [classwrapper,fit=(base)(End)] {};
\node (classname1) [classlbl] at (cw1.west) {Contractor};
\coordinate (marginR) at ($(classname1.north)+(\textwidth,0)+(-5pt,0)$);

% \node [anchor=east] at (marginR){};
\node (process1) [processwrapper,fit=(cw1)(classname1)(marginR)(base)(p2c)(p3)(End),minimum height=5.3cm] {};
\draw (classname1.south east|-process1.north) -- (classname1.south west|-process1.south);

%=====================
% PRINCIPAL SIDE
%=====================
\begin{scope}[yshift=175,xshift=-2.2cm]
\matrix (basep) [draw=none,
  column sep=5pt,row sep=10pt,
] {
  
\node (startp) [StartEvent] {}; 
  & [.05\textwidth] \node (gate1p) [ExclusiveGateway] {};\\
  &\node (gate2p) [ExclusiveGateway]{};\\
};

%-------GRAPH DEFINITION----- 
% \node (p2p) [processEvent] at ($(gate1p.south)!.5!(gate2p.south)+(0,-20pt)$) {New\\Conditions?};
\node (pp1)[processEvent,text width=35,below right=of gate2p,xshift=-.6cm,yshift=-.1cm]{Analyse\\New Conditions};
\node (P2C)[processEvent,text width=25,right=of pp1,xshift=.4cm]{Send\\Decision};
\node (gate3p) [ExclusiveGateway, right =of gate2p,xshift=2.4cm]{};
\node (gate4p) [ParallelGateway,right =of gate3p,xshift=-.3cm]{};
\node (p3)[processEvent,text width=25,above right=of gate4p,xshift=-.5cm]{Amend\\Contract};
\node (p4) [processEvent,text width=25,below right=of gate4p,xshift=-.5cm]{Pay\\Costs};
\node (gate5p) [ParallelGateway,right =of gate4p,xshift=.6cm]{};
\node (e2)[EndEvent,right=of gate5p,xshift=-.5cm]{};

%---- LINES -------
\draw [l] (startp) -- (gate1p);
\draw [l] (gate1p)-- node [lbl,swap,xshift=.1cm,yshift=.2cm]{Major}(gate2p);
\draw [l] (gate2p) |- (pp1);
\draw [l] (pp1) -- (P2C);
\draw [l] (P2C) -- (gate3p);
\draw [l] (gate2p) -- (gate3p);
\draw [l] (gate1p) -| (gate3p);
\draw [l] (gate3p) -- (gate4p);
\draw [l] (gate4p) |- (p3);
\draw [l] (gate4p) |- (p4);
\draw [l] (p3) -| (gate5p);
\draw [l] (p4) -| (gate5p);
\draw [l] (gate5p) -- (e2);

%---- LABELS------
\node [lbl,anchor=west,align=left,yshift=.2cm,xshift=-.2cm] at (gate1p.north) {Type};
\node [lbl,anchor=west,align=left,yshift=-.2cm,xshift=4cm] at (gate1p.north) {Minor};
\node [lbl,anchor=west,align=left,yshift=-.2cm,xshift=2cm] at (gate2p.north) {No};
\node [lbl,anchor=west,align=left,yshift=-.6cm,xshift=.3cm] at (gate2p.north) {New\\Conditions?};
\node [lbl,anchor=west,align=left,yshift=-1.1cm,xshift=-.8cm] at (gate2p.east) {Yes};
\node [lbl,below=of pp1,text width=45,yshift=.3cm,xshift=-.6cm]{Seek Approval};
\node [lbl,anchor=north] at (startp.south) {Start};
\node [lbl,anchor=north] at (e2.south) {End};

%----- WRAPPER---- 
\node (cw2) [classwrapper,fit=(basep)(e2),minimum height=5.2cm] {};
\node (classname2) [classlbl] at (cw2.west) {Principal};
\coordinate (marginR2) at ($(classname2.north)+(.95\textwidth,0)+(-5pt,0)$);
\node (process2) [processwrapper,fit=(cw2)(classname2)(marginR2)] {};
\draw (classname2.south east|-process2.north) -- (classname2.south west|-process2.south);
\end{scope}

\coordinate (m1) at ($(pp1.south)!.5!(p2c.north)$);
\draw [l,dashed] (p2c) |- node [whitecir,pos=0] {} (m1) -| (pp1) ;

\coordinate (m2) at (PP4.south|-m1);
\draw [l,dashed] ($(P2C.south)!.45!(P2C.south)$) -- node [whitecir,pos=0] {} (m2)-- (PP4);


\draw [l,dashed,<-] (start) -- (start.north|-process2.south) node [whitecir] {} ;
\end{tikzpicture}
}

\endinput


==> images/designTime/frag2_wfnet.tex <==
%!TEX root = ../paper.tex

{
\begin{tikzpicture}[
	EventNode/.style={eventNode},
	GatewayNode/.style={gatewayNode},
	PlaceNode/.style={inner sep=4.5pt,circle,draw},
	TransitNode/.style={basicProcessNode,inner sep=0pt,draw,minimum height=1.6em},
	taskId/.style={draw=none,font=\scriptsize,text centered,inner sep=0pt,xshift=-6pt,yshift=2pt},
	l/.style={->,rounded corners=0pt,shorten >=0pt,shorten <=0pt},
]

\matrix [
	column sep=12pt,row sep=2pt,
] {
& & \node (p11) [PlaceNode] {} ;
	& & \node (orJoin1) [TransitNode,WFnetOrJoinsSplit] {} ; 
	& \node (p12) [PlaceNode] {} ;
	& \node (orJoin2) [TransitNode,WFnetOrJoinsSplit] {} ; 
	& \node (p13) [PlaceNode] {} ; \\
& & & & \node (p21) [PlaceNode] {} ; 
	& & \node (p22) [PlaceNode] {} ; 
	& & \node (t5) [TransitNode,WFnetOrJoin,label={[taskId]:$\task[5]$}] {} ; \\
& \node (p31) [PlaceNode] {} ;
	& \node (t2) [TransitNode,WFnetOrSplit,label={[taskId]:$\task[2]$}] {} ; 
	& \node (p32) [PlaceNode] {} ;
	& \node (t3) [TransitNode,WFnetOrSplit,label={[taskId]:$\task[3]$}] {} ; 
	& \node (p33) [PlaceNode] {} ;
	& \node (t4) [TransitNode,WFnetOrSplit,label={[taskId]:$\task[4]$}] {} ; 
	& \node (p34) [PlaceNode] {} ;
	& \node (p35) [PlaceNode] {} ; \\
\node (start) [EventNode,StartEvent,label={[taskId,xshift=6pt,yshift=1.5pt]:source}] {} ;  
\node [fill=black,inner sep=1pt,circle] {} ;
	& \node (t1) [TransitNode,WFnetAndSplit,label={[taskId]:$\task[1]$}] {} ;
	& \node (p41) [PlaceNode] {} ;
	& & & & & 
	& \node (andJoin1) [TransitNode,WFnetAndJoin,label={[taskId]:$\task[6]$}] {} ; 
	& \node (end) [EventNode,EndEvent,label={[taskId,xshift=6pt,yshift=1.5pt]:sink}] {} ;  \\
};

\foreach \n [remember=\n as \lastn (initially p11)] in {orJoin1,p12,orJoin2,p13} {
	\draw [l] (\lastn) -- (\n) ;
}

\foreach \n [remember=\n as \lastn (initially p31)] in {t2,p32,t3,p33,t4,p34} {
	\draw [l] (\lastn) -- (\n) ;
}

\foreach \n [remember=\n as \lastn (initially start)] in {t1,p41,andJoin1,end} {
	\draw [l] (\lastn) -- (\n) ;
}

\foreach \n [remember=\n as \lastn (initially t3)] in {p21,orJoin1} {
	\draw [l] (\lastn) -- (\n) ;
}

\foreach \n [remember=\n as \lastn (initially t4)] in {p22,orJoin2} {
	\draw [l] (\lastn) -- (\n) ;
}

\draw [l] (t1) -- (p31) ;
\draw [l] (t2) -- (p11) ;
\draw [l] (p13) -| (t5) ;
\draw [l] (p34) |- (t5) ;
\draw [l] (t5) -- (p35) ;
\draw [l] (p35) -- (andJoin1) ;

\end{tikzpicture}
}

\endinput


==> images/designTime/task.tex <==
%!TEX root = ../manuscript.tex


{
\begin{tikzpicture}[
ProcessNode/.style={processNode,inner sep=2pt},
unusedDeliverables/.style={decorate,decoration={coil,aspect=0,pre=lineto,pre length=1pt,post length=3pt}},
resourcesLine/.style={auto,decorate,decoration={shape backgrounds,shape=dart,shape sep=5pt},shape border rotate=180},
linelabel/.style={LineLabel},
]

\node (rules) [font=\scriptsize,draw,inner sep=4pt,rounded corners=3pt] {Rules} ;
\node (task) [anchor=south,inner sep=3pt] at ($(rules.north)+(0pt,2pt)$) {$Task_i$} ;

\node (task-1) [ProcessNode,fit=(task)(rules),minimum width=5.4em,inner sep=3pt] {};


\coordinate (task-0) at ($(task-1.west)+(-6em,0)$) ;
\coordinate (task-2) at ($(task-1.east)+(6em,0)$) ;

\foreach \n [count=\c, remember=\c as \lastc (initially 0)] in {i-1} {
  \draw [->,dashed,yshift=-10pt] ($(task-\lastc.east)+(0,5pt)$) to [out=20,in=160] ($(task-\c.west)+(0,5pt)$)
  	;
  \draw [->] (task-\lastc) -- (task-\c)
    node (effect-\c) [linelabel,swap,midway,yshift=3.0em] {$\effect[\n][1..n_{\n}]$} 
    ;
}

\foreach \n/\lastc/\c in {i/1/2} {
  \draw [->,dashed,yshift=-10pt] ($(task-\lastc.east)+(0,-5pt)$) to [out=340,in=200] ($(task-\c.west)+(0,-5pt)$)
    ;
  \draw [->] (task-\lastc) -- (task-\c)
    node (effect-\c) [linelabel,swap,midway,yshift=-1.6em] {$\effect[\n][1..n_{\n}]$} 
    ;
}


\draw [->,unusedDeliverables] (task-1) 
  -- ++ (4.95em,3em) 
    node [linelabel,inner sep=1pt,auto,anchor=south,xshift=-0em] {$\deliverable[i][1..d_{i}]$}
    ;

\draw [<-,resourcesLine] (task-1.south) + (0,-5pt) 
  -- ++ (0,-1.9em) 
    node [linelabel,anchor=north,inner sep=2pt,yshift=5pt] {$\resource[i][1..r_{i}]$}
    ;

\end{tikzpicture}
% \medskip
}


\endinput



==> images/designTime/testProcess.tex <==
%!TEX root = ../paper.tex

{
\begin{tikzpicture}[
ProcessNode/.style={processNode,font=\scriptsize,rounded corners=3pt,text width=3em,minimum height=2.8em},
GatewayNode/.style={gatewayNode},
EventNode/.style={eventNode},
placeHolderNode/.style={draw=none,minimum width=#1},
taskId/.style={draw=none,font=\scriptsize,text centered,inner sep=3pt},
lbl/.style={Label,font=\tiny},
conditionLabel/.style={lbl,yshift=-1.9em,text width=30,anchor=north,below},
decisionLabel/.style={lbl,text centered},
l/.style={->,rounded corners=5pt,shorten >=0pt,shorten <=0pt},
]

\matrix (base) [draw=none,
  column sep=7pt,row sep=1.5em,
] {
&&&& \node (g1) [GatewayNode,ExclusiveGateway] {} ; \\
  % & \node (end1) [EndEvent,label={[lbl]below:End}] {} ; \\
\node (start) [StartEvent,label={[lbl]below:Start}] {} ; 
  & \node (sendTaxInvoice) [ProcessNode,text width=5em] {Send tax invoice in 30 days} ;
  & \node (g2) [GatewayNode,ExclusiveGateway] {} ;
  & \node (getPayment1) [ProcessNode] {get payment} ;
  & \node (g3) [GatewayNode,ExclusiveGateway] {} ;
  & \node (g4) [GatewayNode,ParallelGateway] {} ;
  & \node (placeHolder) [text width=5.5em] {} ;
  % & \node (computeComplianceDegree) [ProcessNode,text width=5.5em] {Compute\\ compliance degree} ;
  & \node (g5) [GatewayNode,ParallelGateway] {} ;
  & \node (getPayment2) [ProcessNode] {get payment} ; 
  & \node (determineAction) [ProcessNode] {determine action} ;
  & \node (notifyCustomer) [ProcessNode] {notify customer} ;
  & \node (g6) [GatewayNode,ExclusiveGateway] {} ;
  & \node (end2) [EndEvent,label={[lbl]below:End}] {} ; \\
% &&&&& & \node (calculateComp) [ProcessNode,text width=5.5em] {Calculate\\ degree of comp} ; \\
% && & \node (specialAction) [ProcessNode,yshift=.5em] {Special action} ; \\
  % & \node (g6) [GatewayNode,ExclusiveGateway] {} ;
  % && \node (notifyCustomer) [ProcessNode] {notify customer} ;
  % && \node (determineAction) [ProcessNode] {determine action} ; \\
% &&&& \node (end2) [EndEvent,label={[lbl]below:End}] {} ; \\
};

\node (computeComplianceDegree) [ProcessNode,text width=5.5em,yshift=1.9em] at (placeHolder) {Compute\\ compliance degree} ;
\node (calculateComp) [ProcessNode,text width=5.5em,yshift=-1.9em] at (placeHolder) {Calculate\\ degree of comp} ;

\node (specialAction) [ProcessNode,anchor=north west,yshift=-1.1em] at (getPayment1.south west) {Special action} ; 


\foreach \n/\l [remember=\n as \lastn (initially start)] in {sendTaxInvoice/,g2/,getPayment1/,
    g3/,g4/} {
  \draw [l,->] (\lastn) -- node [lbl] {\l} (\n) ;
}

\foreach \n/\l [remember=\n as \lastn (initially g5)] in {getPayment2/,determineAction/,notifyCustomer/,g6/,end2/} {
  \draw [l,->] (\lastn) -- node [lbl] {\l} (\n) ;
}

\draw [l,->] (g2) |- (g1) ;
\draw [l,->] (g1) -| (g6) ;
% \draw [l,->] (g1) -- (end1) ;

\draw [l,->] (g2) |- (specialAction) ;
\draw [l,->] (specialAction) -| (g6) ;

\draw [l,->] (g3) -- (g1) ;

\draw [l,->] (g4) |- (computeComplianceDegree) ;
\draw [l,->] (computeComplianceDegree) -| (g5.north) ;

\draw [l,->] (g4) |- (calculateComp) ;
\draw [l,->] (calculateComp) -| (g5) ;

\end{tikzpicture}
}

\endinput

